On the Evaluation and Real-World Usage Scenarios of Deep Vessel Segmentation for Retinography

We identify and address three research gaps in the field of vessel segmentation for funduscopy. The first focuses on the task of inference on high-resolution fundus images for which only a limited set of ground-truth data is publicly available. Notably, we highlight that simple rescaling and padding or cropping of lower resolution datasets is surprisingly effective. Additionally we explore the effectiveness of semi-supervised learning for better domain adaptation. Our results show competitive performance on a set of common public retinal vessel datasets using a small and light-weight neural network. For HRF, the only very high-resolution dataset currently available, we reach new state-of-the-art performance by solely relying on training images from lower-resolution datasets. The second topic concerns evaluation metrics. We investigate the variability of the F1-score on the existing datasets and report results for recent SOTA architectures. Our evaluation show that most SOTA results are actually comparable to each other in performance. Last, we address the issue of reproducibility by open-sourcing our complete pipeline.

==> chase.tex <==
\begingroup
\setlength\tabcolsep{4pt} % default value: 6pt
\begin{table}[htb]
\scriptsize
\caption{
Comparison with previous works on CHASE\_DB1
}
\label{tab:chase}
\begin{center}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                     &        & \multicolumn{5}{c}{Target: CHASE\_DB1}                                     \\ \cmidrule(lr){3-7}
Method                                               & Year   & F1            & Acc             & Pr                & Re (Se)           & Sp              \\ \midrule
2nd human observer                                   &        & 0.7686          & 0.9538          & -                 & -                 & -               \\
\textbf{Unsupervised}                                &        &                 &                 &                   &                   &                 \\ \hline
Azzopardi et al.~\cite{azzopardi_trainable_2015}     & 2015   & -               & 0.9387          & -                 & 0.7585            & 0.9587          \\
Zhang et al.~\cite{zhang_robust_2016}                & 2016   & -               & 0.9452          & -                 & 0.7626            & 0.9661          \\
\textbf{Supervised}                                  &        &                 &                 &                   &                   &                 \\ \hline
Fraz et al.~\cite{fraz_ensemble_2012}*      & 2012   & 0.7566          & 0.9469          & 0.7415            & 0.7224            & 0.9711          \\
Jin et al.~\cite{jin_dunet_2019}                    & 2019   & 0.7883          & 0.9610          & 0.7630            & 0.8155            & 0.9752          \\
Laibacher et al.~\cite{laibacher_m2u_2018}*  & 2018   & 0.8006          & -               & -                 & -                 & -               \\
Li et al.~\cite{li_cross-modality_2016}              & 2016   & -               & 0.9581          & -                 & 0.7507            & 0.9793          \\
Orlando et al.~\cite{orlando_discriminatively_2017}  & 2017   & 0.7332          & -               & 0.7438            & 0.7277            & 0.9712          \\
Roychowdhury et al.~\cite{roychowdhury_blood_2015}   & 2015   & -               & 0.9530          & -                 & 0.7201            & 0.9824          \\
Yan et al.~\cite{yan_joint_2018}                     & 2018   & -               & 0.9610          & -                 & 0.7633            & 0.9809          \\
DRIU~\cite{maninis_deep_2016} (our impl.)*            &        & \textbf{0.8114} & \textbf{0.9716} & \textbf{0.8068}	  & 0.8160	          & \textbf{0.9842} \\
\textbf{M2U-Net CHASE\_DB1}                          &        & 0.8022          & 0.9704          & 0.7985	          & 0.8086	          & 0.9835          \\ \hline
\textbf{M2U-Net COVD --}                           &        & 0.7884          & 0.9678          & 0.7710	          & 0.8095	          & 0.9807          \\
\textbf{M2U-Net COVD -- SSL}                      &        & 0.7988          & 0.9694          & 0.7819	          & \textbf{0.8189}	  & 0.9816          \\ \hline 
\multicolumn{7}{l}{*Same train-test split as adopted in this work}  \\ \bottomrule
\end{tabular}
\end{center}
\end{table}
\endgroup

==> drive.tex <==
\begingroup
\setlength\tabcolsep{4pt} % default value: 6pt

\begin{table}[htb]
\scriptsize
%\setlength\tabcolsep{2pt}
\caption{Comparison with previous works on DRIVE}
\label{tab:drive}
\begin{center}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                    &      & \multicolumn{5}{c}{Target: DRIVE (584x565)}                                             \\ \cmidrule(lr){3-7}
Method                                              & Year & F1            & Acc             & Pr                & Re (Se)           & Sp                    \\ \hline
2nd human observer                                  &      & 0.7931          & 0.7881          & 0.8072            & 0.7796            & 0.9717                \\
\textbf{Unsupervised}                               &      & -               &                 & -                 & -                 & -                     \\       
Bibiloni et al.~\cite{bibiloni_real-time_2018}      & 2018 & 0.7521          & 0.938           & 0.786             & 0.721             & 0.970                 \\      
\textbf{Supervised}                                 &      &                 &                 &                   &                   &                       \\ \hline     
Fraz et al.~\cite{fraz_ensemble_2012}               & 2012 & 0.7929          & 0.9480          & \textbf{0.8532}   & 0.7406            & 0.9807                \\
Jin et al.~\cite{jin_dunet_2019}                   & 2019 & 0.8237          & 0.9566          & 0.8529            & 0.7963            & 0.9800                \\ 
Laibacher et al.~\cite{laibacher_m2u_2018}          & 2018 & 0.8091          & -               & -                 & -                 & -                     \\ 
Li et al.~\cite{li_cross-modality_2016}             & 2016 & -               & 0.9527          & -                 & 0.7569            & \textbf{0.9816}       \\    
Liskowski et al.~\cite{liskowski_segmenting_2016}   & 2016 & -               & 0.9535          & -                 & 0.7811            & 0.9807                \\    
Maninis et al.~\cite{maninis_deep_2016}             & 2016 & \textbf{0.8220} & -               & -                 & -                 & -                     \\   
Marin et al.~\cite{marin_new_2011}                  & 2011 & 0.8134          & 0.9452          & 0.9582            & 0.7067            & 0.9801                \\  
Orlando et al.~\cite{orlando_discriminatively_2017} & 2017 & 0.7857          & -               & 0.7854            & 0.7897            & 0.9684                \\
Yan et al.~\cite{yan_joint_2018}                    & 2018 & 0.8183          & 0.9529          & 0.8124            & \textbf{0.8242}   & 0.9720                \\ 
Zhao et al.~\cite{zhao_supervised_2019}             & 2019 & 0.7882          & -               & -                 & -                 & -                     \\ 
\textbf{M2U-Net DRIVE}                              &      & 0.8030         & \textbf{0.9619} & 0.8103	        & 0.8000	        & 0.9797                \\ \hline
\textbf{M2U-Net COVD --}                          &      & 0.7885         & 0.9592          & 0.7990	        & 0.7824	        & 0.9787                \\
\textbf{M2U-Net COVD -- SSL}                     &      & 0.7913         & 0.9598          & 0.8016	        & 0.7862	        & 0.9789                \\ \hline 
\multicolumn{7}{l}{All supervised methods use the same train-test split}  \\ \bottomrule
\end{tabular}
\end{center}
\end{table}
\endgroup

==> hrf.tex <==
\begingroup
\setlength\tabcolsep{4pt} % default value: 6pt
\begin{table}[htpb]
\scriptsize
%\setlength\tabcolsep{1.5pt}
\caption{
Comparison with previous works on HRF
}
\label{tab:hrf}
\begin{center}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                                &   & \multicolumn{5}{c}{Target: HRF (2336x3504)}                                                                      \\ \cmidrule(lr){3-7}
Method                                                          & Year & F1            & Acc              & Pr                & Re (Se)           & Sp                   \\ \hline
\textbf{Unsupervised}                                           &      &                 &                  &                   &                   &                      \\ \hline
Annunziata et al.~\cite{annunziata_leveraging_2016}             & 2016 & 0.7578          & 0.9581           & 0.8089            & 0.7128            & 0.9836               \\
Budai et al.~\cite{budai_robust_2013}                           & 2013 & -               & 0.9610           & -                 & 0.669             & 0.985                \\
Odstrcilik et al.~\cite{odstrcilik_retinal_2013}                & 2013 & 0.7324          & 0.9494           &                   & 0.7741            & 0.9669               \\
Zhang et al.~\cite{zhang_robust_2016}                           & 2016 & -               & 0.9556           & -                 & 0.7978            & 0.9710               \\
\textbf{Supervised}                                             &      &                 &                 &                    &                   &                      \\  \hline
Orlando et al.~\cite{orlando_discriminatively_2017}*   & 2017 & 0.7158          & -                & 0.6630            & 0.7874            & 0.9584               \\
Yan et al.~\cite{yan_joint_2018}*                     & 2018 & 0.7212          & 0.9437           & 0.6647            & 0.7881            & 0.9592               \\
Laibacher et al.~\cite{laibacher_m2u_2018}*            & 2018 & 0.7814          & 0.9635           & -                 & -                 & -                    \\ 
Jin et al.~\cite{jin_dunet_2019}*                              & 2019 & 0.7988          & 0.9651           &  \textbf{0.8593}            & 0.7464                  & \textbf{0.9874} \\
Zhao et al.~\cite{zhao_supervised_2019}                         & 2019 & 0.7659          & -                & -                 & -                 & -                    \\        
DRIU~\cite{maninis_deep_2016} (our impl.)*                       &      & 0.7865          & 0.9646           & 0.7863	        & 0.7868            & 0.9806               \\                               
\textbf{M2U-Net HRF}                                            &      & 0.7800          & 0.9641           & 0.7798	        & 0.7880            & 0.9798               \\ \hline 
\textbf{M2U-Net COVD -}                                       &      & \textbf{0.8020} & \textbf{0.9669}  & 0.7889	& \textbf{0.8188}   & 0.9802               \\
\textbf{M2U-Net COVD - SSL}                                   &      & 0.7972          & 0.9659           & 0.7898	        & 0.8021            & \textbf{0.9807}      \\ \hline 
\multicolumn{7}{l}{*Same train-test split as adopted in this work}  \\ \bottomrule
\end{tabular}
\end{center}
\end{table}
\endgroup

==> iostar.tex <==
\begingroup
\setlength\tabcolsep{4pt} % default value: 6pt
\begin{table}[htbp]
\scriptsize
\caption{
Comparison with previous works on IOSTAR
}
\label{tab:iostar}
\begin{center}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                                              &         & \multicolumn{5}{c}{Target: IOSTAR (1024x1024)}                                \\ \cmidrule(lr){3-7}
Method                                                                        & Year    & F1            & Acc             & Pr                & Re (Se)           & Sp                \\ \hline
\textbf{Supervised}                                                           &         &                 &                 &                   &                   &                   \\ \hline
Abbasi-Sureshjani et al.~\cite{abbasi_iostar_2015}  & 2015    & -               & 0.9501          &                   & 0.7863            & 0.9747            \\
Meyer et al.~\cite{meyer_deep_2017}*                                & 2017    & -               & 0.9695          & -                 & 0.8038            & 0.9801            \\
Zhang et al.~\cite{zhang_robust_2016}                                         & 2016    & -               & 0.9514          & -                 & 0.7545            & 0.9740            \\
Zhao et al.~\cite{zhao_supervised_2019}                                       & 2019    & 0.7707          & -               & -                 & -                 & -                 \\
DRIU~\cite{maninis_deep_2016} (our impl.)                                     &         & \textbf{0.8273} & \textbf{0.9721} & \textbf{0.8173}	& \textbf{0.8376}	& \textbf{0.9839}   \\                               
\textbf{M2UNet IOSTAR}                                                        &         & 0.8173          & 0.9708          & 0.8081      	    & 0.8311	        & 0.9831            \\ \bottomrule
\textbf{M2U-Net COVD --}                                                    &         & 0.7928          & 0.9665          & 0.7755	        & 0.8161	        & 0.9798            \\
\textbf{M2U-Net COVD -- SSL}                                               &         & 0.7845          & 0.9644          & 0.7544	        & 0.8221	        & 0.9770            \\ \hline 
\multicolumn{7}{l}{*Same train-test split as adopted in this work}  \\ \bottomrule
\end{tabular}
\end{center}
\end{table}
\endgroup

==> stare.tex <==
\begingroup
\setlength\tabcolsep{4pt} % default value: 6pt
\begin{table}[htb]
\scriptsize
%\setlength\tabcolsep{1.5pt}
\caption{
Comparison with previous works on STARE
}
\label{tab:stare}
\begin{center}
\begin{tabular}{@{}ccccccc@{}}
\toprule
                                                        &            & \multicolumn{5}{c}{Target: STARE (605x700)}                                      \\ \cmidrule(lr){3-7}
Method                                                  &  Year      & F1            & Acc                 & Pr                & Re (Se)            & Sp                   \\ \hline
2nd human observer                                      &            & -               & 0.9347              & 0.6432            & \textbf{0.8955}    & 0.9382               \\  
\textbf{Unsupervised}                                   &            & -               & -                   & -                 & -                  & -                    \\      
Bibiloni et al.~\cite{bibiloni_real-time_2018}          & 2018       & 0.752           & 0.938               & 0.786             & 0.721              & 0.970                \\     
\textbf{Supervised}                                     &            &                 &                     &                   &                    &                      \\ \hline     
Fraz et al.~\cite{fraz_ensemble_2012}                   & 2012       & 0.7747          & 0.9347              & 0.7956            & 0.7548             & 0.9763               \\
Jin et al.~\cite{jin_dunet_2019}                       & 2019       & 0.8143          & 0.9641              & 0.8777            & 0.7595             & \textbf{0.9878}     \\
Li et al.~\cite{li_cross-modality_2016}                 & 2016       & -               & 0.9628              & -                 & 0.7726             & 0.9844               \\        
Maninis et al.~\cite{maninis_deep_2016}*       & 2016       & \textbf{0.831}  & -                   & -                 & -                  & -                    \\     
Marin et al.~\cite{marin_new_2011}                      & 2011       & 0.8080          & 0.9526              & \textbf{0.9659}   & 0.6944             & 0.9819               \\     
Orlando et al.~\cite{orlando_discriminatively_2017}     & 2017       & 0.7644          & -                   & 0.7740            & 0.7680             & 0.9738               \\
Yan et al.~\cite{yan_joint_2018}                        & 2018       & -               & 0.9612              & -                 & 0.7581             & 0.9846               \\
Zhao et al.~\cite{zhao_supervised_2019}*       & 2019       & 0.7960          & -                   & -                 & -                  & -                    \\ 
\textbf{M2U-Net STARE}                                  &            & 0.8150          & 0.9727              & 0.8090	        & 0.8257	         & 0.9848               \\ \hline
\textbf{M2U-Net COVD --}                              &            & 0.8117          & 0.9724              & 0.8128	        & 0.8114	         & 0.9851               \\
\textbf{M2U-Net COVD -- SSL}                         &            & 0.8196          & \textbf{0.9734}     & 0.8164   	        & 0.8282	         & 0.9847               \\ \hline 
\multicolumn{7}{l}{*Same train-test split as adopted in this work}  \\ \bottomrule
\end{tabular}
\end{center}
\end{table}
\endgroup
